Fast Correlation Heating in Moderately Coupled Electron-Ion Plasmas

If the electrons in a plasma are suddenly heated, the resulting change in Debye shielding causes the ion kinetic energy to quickly increase. For the first time, this correlation heating, which is much faster than collisional energy exchange, is rigorously derived for a moderately coupled, electron-ion plasma. The electron-ion mass ratio is taken to be the smallest parameter in the BBGKY hierarchy, smaller even than the reciprocal of the plasma parameter. This ordering differs from conventional kinetic theory by making the electron collision rates faster than the ion plasma frequency, which allows stronger coupling and makes the ion heating a function only of the total energy supplied to the electrons. The calculation uses known formulas for correlations in a two-temperature plasma, for which a new, elementary derivation is presented. Suprathermal ions can be created more rapidly by this mechanism than by ion-electron Coulomb collisions. This means that the use of a femtosecond laser pulse could potentially help to achieve ignition in certain fast ignition approaches to ICF.

==> tikzlibraryavoidpath.code.tex <==
% Copyright 2015 by Kpym
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
\typeout{tikz-avoidpath v1.0}

% some additional libraries used by this one
\usetikzlibrary{calc,math,decorations.markings,patterns}

% style for arrows on the path
% Usage :
%  [with arrows=35mm] put arrows every 35mm
%  [with arrows at positions={35mm,70mm,140mm}] put arrows at 35mm,70mm,140mm
% -----------------------------------------------------------
\tikzset{
  with arrows/.style={
    decoration={ markings,
      mark=between positions #1 and .999 step #1 with {\arrow{stealth}}
    }, postaction={decorate}
  }, with arrows/.default=13mm,
  with arrow at/.style={
    decoration={ markings,
      mark=at position #1 with {\arrow{stealth}}
    }, postaction={decorate}
  }, with arrows/.default=13mm,
  with arrows at positions/.style={
   with arrow at/.list={#1}
  }
}

% style to draw reversed circle (helpfull when filling, to not fill inside)
% Usage :
%   circle[reversed with radius=1cm]
% -----------------------------------------------------------
\tikzset{
  reversed with radius/.style={
    x radius=#1,
    y radius=-#1,
  }
}

% macros to use tikzmath inside 'to path'
% -----------------------------------------------------------
\newcommand\tikzmathextra[1]{\pgfextra{\tikzmath{#1}}}
\newcommand\insertpath[1]{\pgfkeys{/tikz/insert path={#1}}}

% macros for data dependancies
% Usage :
%  .pgfmathparse in=\macroname is like ".store in", but mathparse it first
%  .pgfmathsync to=\macroname{<formula>} every time the key is set, the <formula> is mathparsed and stored in \macroname
% -----------------------------------------------------------
\pgfkeys{
  /handlers/.pgfmathparse in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\pgfmathsetmacro#1{##1}\ifpgfmathunitsdeclared\edef#1{#1 pt}\else\edef#1{#1 cm}\fi},
  /handlers/.pgfmathsync to/.code 2 args=\pgfkeysalso{\pgfkeyscurrentpath/.append code=\pgfmathparse{#2}\edef\result{\pgfmathresult}\ifpgfmathunitsdeclared\providecommand#1{\result pt}\else\providecommand#1{\result cm}\fi}
}

% precision : pgfmathparse is not very precise we consides 0 <=> < \avoidpointprecision
%  in particular two point are considered identical if the distance is < \avoidpointprecision
%  for the same reason \avoidonaxeprecision is used to check if the pole is on the line (\tikztostart)--(\tikztotarget)
% -----------------------------------------------------------
\tikzset{
  /avoid/.cd,
  point precision/.store in=\avoidpointprecision,
  on axe precision/.store in=\avoidonaxeprecision,
  precision/.style={point precision=#1,on axe precision=#1},
  precision=.7pt % the initial precision
}

% main to path
% -----------------------------------------------------------
\tikzset{
  % styles to set the variables
  /avoid/.cd,
    pole/.store in=\avoidpole,
    radius/.pgfmathparse in=\avoidradius,
    radius/.pgfmathsync to=\avoidneck{\avoidradius},
    neck/.pgfmathparse in=\avoidneck,
    neck/.pgfmathsync to=\avoidradius{\avoidneck},
    side/.store in=\avoidside, side=0,
    left/.style={side=1},
    right/.style={side=-1},
  /tikz/.cd,
  % the main style
  avoid/.style={/avoid/.cd,#1,/tikz/.cd, % set the varaibles
    to path={
      \tikzmathextra{
        point \p; % points
        real \a; % angles (in degree)
        \p{start} = (\tikztostart);
        \p{target} = (\tikztotarget);
        \p{pole} = \avoidpole; % \avoidpole is like (A) or (1,0)
        \p{projection} = (\p{start})!(\p{pole})!(\p{target});
        if (abs(\px{projection}-\px{pole}) + abs(\py{projection}-\py{pole})) < \avoidonaxeprecision then {
          % if the pole is on the main axe (left and right options are valid)
          \p{first base} = (\p{projection})!\avoidradius!(\p{start});
          \a{start} = atan2(\py{start}-\py{projection},\px{start}-\px{projection});
          if \avoidside >= 0 then {
            \a{target} = \a{start}-180; % left
          } else {
            \a{target} = \a{start}+180; % right
          };
          if (abs(\px{first base}-\px{start}) + abs(\py{first base}-\py{start})) > \avoidpointprecision then {
            {\insertpath{-- (\p{first base})}};
          };
          {\insertpath{arc(\a{start}:\a{target}:\avoidradius)}};
        } else {
          % if pole outside of the main axe (left and right options are useless)
          \sameasneck = abs(veclen(\px{target}-\px{start},\py{target}-\py{start})-\avoidneck) < \avoidpointprecision;
          if \sameasneck then {
            % if |\p{target}-\p{start}| ~= \avoidneck
            \p{first base} = (\p{start});
            \p{second base} = (\p{target});
          }
          else{
            \p{first base} = (\p{projection})!\avoidneck/2!(\p{start});
            \p{second base} = (\p{projection})!\avoidneck/2!(\p{target});
          };
          \p{neck vector} = (\p{pole})!sqrt((\avoidradius)^2-(\avoidneck/2)^2)!(\p{projection})-(\p{projection});
          \p{first on circle} = (\p{first base}) + (\p{neck vector});
          \p{second on circle} = (\p{second base}) + (\p{neck vector});
          \a{start} = atan2(\py{first on circle}-\py{pole},\px{first on circle}-\px{pole});
          \a{target} = atan2(\py{second on circle}-\py{pole},\px{second on circle}-\px{pole});
          if abs(\a{start}-\a{target}) < 180 then {
            if \a{start} < \a{target} then {
              \a{start} = \a{start} + 360;
            }
            else {
              \a{target} = \a{target} + 360;
            };
          };
          if not \sameasneck then {
            {\insertpath{-- (\p{first base})}};
          };
          {\insertpath{-- (\p{first base}) -- (\p{first on circle}) arc(\a{start}:\a{target}:\avoidradius)}};
          if not \sameasneck then {
            {\insertpath{-- (\p{second base})}};
          };
        };
      }% end tikzmathextra
      --(\tikztotarget) \tikztonodes
    }% end to path
  }% end avoid/.style
}





